Terrestrial Very-Long-Baseline Atom Interferometry: Summary of the Second Workshop

This summary of the second Terrestrial Very-Long-Baseline Atom Interferometry (TVLBAI) Workshop provides a comprehensive overview of our meeting held in London in April 2024, building on the initial discussions during the inaugural workshop held at CERN in March 2023. Like the summary of the first workshop, this document records a critical milestone for the international atom interferometry community. It documents our concerted efforts to evaluate progress, address emerging challenges, and refine strategic directions for future large-scale atom interferometry projects. Our commitment to collaboration is manifested by the integration of diverse expertise and the coordination of international resources, all aimed at advancing the frontiers of atom interferometry physics and technology, as set out in a Memorandum of Understanding signed by over 50 institutions.

==> authorlist.tex <==
% Auto-generated author list for LaTeX document
% Include this file in your LaTeX document using \input{authorlist.tex}

% Author List
\author[1]{Adam~Abdalla,}
\author[2]{Mahiro~Abe,}
\author[3]{Sven~Abend,}
\author[3]{Mouine~Abidi,}
\author[4,5,6,*]{Monika~Aidelsburger,}
\author[3]{Ashkan~Alibabaei,}
\author[7,*]{Baptiste~Allard,}
\author[8]{John~Antoniadis,}
\author[9,*]{Gianluigi~Arduini,}
\author[10]{Nadja~Augst,}
\author[11]{Philippos~Balamatsias,}
\author[12,13]{Antun~Bala\v{z},}
\author[14]{Hannah~Banks,}
\author[2]{Rachel~L.~Barcklay,}
\author[15]{Michele~Barone,}
\author[16]{Michele~Barsanti,}
\author[17]{Mark~G.~Bason,}
\author[18,19]{Angelo~Bassi,}
\author[20,*]{Jean-Baptiste~Bayle,}
\author[21,*]{Charles~F.~A.~Baynham,}
\author[22]{Quentin~Beaufils,}
\author[7]{Sélyan~Beldjoudi,}
\author[12]{Aleksandar~Beli\'{c},}
\author[23,24,*]{Shayne~Bennetts,}
\author[25]{Jose~Bernabeu,}
\author[26,*]{Andrea~Bertoldi,}
\author[7]{Clara~Bigard,}
\author[27]{N.~P.~Bigelow,}
\author[28]{Robert~Bingham,}
\author[29,30]{Diego~Blas,}
\author[31]{Alexey~Bobrick,}
\author[32]{Samuel~Boehringer,}
\author[12]{Aleksandar~Bogojevi\'{c},}
\author[10,*]{Kai~Bongs,}
\author[33]{Daniela~Bortoletto,}
\author[23,34,35,*]{Philippe~Bouyer,}
\author[10]{Christian~Brand,}
\author[21,33,*,@]{Oliver~Buchmueller,}
\author[36]{Gabriela~Buica,}
\author[9,*]{Sergio~Calatroni,}
\author[7]{Léo~Calmels,}
\author[14]{Priscilla~Canizares,}
\author[26,*]{Benjamin~Canuel,}
\author[36]{Ana~Caramete,}
\author[36]{Laurentiu-Ioan~Caramete,}
\author[18,19]{Matteo~Carlesso,}
\author[37]{John~Carlton,}
\author[2]{Samuel~P.~Carman,}
\author[38]{Andrew~Carroll,}
\author[39,40]{Mateo~Casariego,}
\author[11]{Minoas~Chairetis,}
\author[8,41,42]{Vassilis~Charmandaris,}
\author[43]{Upasna~Chauhan,}
\author[44]{Jiajun~Chen,}
\author[45,46,*]{Maria~Luisa~(Marilù)~Chiofalo,}
\author[45]{Donatella~Ciampini,}
\author[21]{Alessia~Cimbri,}
\author[47,*]{Pierre~Cladé,}
\author[38]{Jonathon~Coleman,}
\author[48]{Florin~Lucian~Constantin,}
\author[21]{Carlo~R.~Contaldi,}
\author[22,*]{Robin~Corgier,}
\author[49]{Bineet~Dash,}
\author[21]{G.J.~Davies,}
\author[21]{Claudia~de~Rham,}
\author[9,*]{Albert~De~Roeck,}
\author[1]{Daniel~Derr,}
\author[43]{Soumyodeep~Dey,}
\author[32,*]{Fabio~Di~Pumpo,}
\author[50,51]{Goran~S.~Djordjevic,}
\author[52]{Babette~D\"obrich,}
\author[21]{Peter~Dornan,}
\author[9,*]{Michael~Doser,}
\author[53]{Giannis~Drougakis,}
\author[54]{Jacob~Dunningham,}
\author[49,55]{Alisher~Duspayev,}
\author[28]{Sajan~Easo,}
\author[56,*]{Joshua~Eby,}
\author[10,32]{Maxim~Efremov,}
\author[38]{Gedminas~Elertas,}
\author[57,*,@]{John~Ellis,}
\author[2]{Nicholas~Entin,}
\author[58,*]{Stephen~Fairhurst,}
\author[59]{Mattia~Fan\`i,}
\author[60]{Farida~Fassi,}
\author[61,62]{Pierre~Fayet,}
\author[36]{Daniel~Felea,}
\author[63]{Jie~Feng,}
\author[64]{Robert~Flack,}
\author[33,*]{Chris~Foot,}
\author[65]{Tim~Freegarde,}
\author[66,67]{Elina~Fuchs,}
\author[3,*]{Naceur~Gaaloul,}
\author[68]{Dongfeng~Gao,}
\author[69]{Susan~Gardner,}
\author[54]{Barry~M.~Garraway,}
\author[22]{Carlos~L.~Garrido~Alzar,}
\author[7,*]{Alexandre~Gauguet,}
\author[1,*]{Enno~Giese,}
\author[70]{Patrick~Gill,}
\author[9]{Gian~F.~Giudice,}
\author[32]{Eric~P.~Glasbrenner,}
\author[71,*]{Jonah~Glick,}
\author[2]{Peter~W.~Graham,}
\author[9]{Eduardo~Granados,}
\author[72]{Paul~F.~Griffin,}
\author[22,29]{Jordan~Gu\'e,}
\author[47,73]{Sa\"{\i}da~Guellati-Khelifa,}
\author[74,*]{Subhadeep~Gupta,}
\author[3]{Vishu~Gupta,}
\author[75]{Lucia~Hackermueller,}
\author[76]{Martin~Haehnelt,}
\author[9]{Timo~Hakulinen,}
\author[66]{Klemens~Hammerer,}
\author[77]{Ekim~T.~Han{\i}meli,}
\author[44,*]{Tiffany~Harte,}
\author[32]{Sabrina~Hartmann,}
\author[21,*]{Leonie~Hawkins,}
\author[22]{Aurelien~Hees,}
\author[3,*]{Alexander~Herbst,}
\author[33,43,*]{Thomas~M.~Hird,}
\author[21,*]{Richard~Hobson,}
\author[2,*]{Jason~Hogan,}
\author[78]{Bodil~Holst,}
\author[43,*]{Michael~Holynski,}
\author[79,*]{Onur~Hosten,}
\author[44]{Chung~Chuan~Hsu,}
\author[80]{Wayne~Cheng-Wei~Huang,}
\author[33]{Kenneth~M.~Hughes,}
\author[28,38]{Kamran~Hussain,}
\author[81]{Gert~H\"utsi,}
\author[82,83,84]{Antonio~Iovino,}
\author[36,85]{Maria-Catalina~Isfan,}
\author[32]{Gregor~Janson,}
\author[86]{Peter~Jegli\v{c},}
\author[87]{Philippe~Jetzer,}
\author[2]{Yijun~Jiang,}
\author[88]{Gediminas~Juzeli\=unas,}
\author[89,*]{Wilhelm~Kaenders,}
\author[90]{Matti~Kalliokoski,}
\author[91]{Alex~Kehagias,}
\author[64]{Eva~Kilian,}
\author[92,*]{Carsten~Klempt,}
\author[21,*]{Peter~Knight,}
\author[93]{Soumen~Koley,}
\author[10]{Bernd~Konrad,}
\author[71,*]{Tim~Kovachy,}
\author[94,95]{Markus~Krutzik,}
\author[96]{Mukesh~Kumar,}
\author[97]{Pradeep~Kumar,}
\author[17,38]{Hamza~Labiad,}
\author[24,80,98,*]{Shau-Yu~Lan,}
\author[22]{Arnaud~Landragin,}
\author[99]{Greg~Landsberg,}
\author[100]{Mehdi~Langlois,}
\author[101]{Bryony~Lanigan,}
\author[102]{Bruno~Leone,}
\author[22]{Christophe~Le~Poncin-Lafitte,}
\author[43]{Samuel~Lellouch,}
\author[103]{Marek~Lewicki,}
\author[43]{Yu-Hung~Lien,}
\author[104,*]{Lucas~Lombriser,}
\author[105,106,*]{Elias~Lopez~Asamar,}
\author[107]{J.Luis~Lopez-Gonzalez,}
\author[44]{Chen~Lu,}
\author[108]{Giuseppe~Gaetano~Luciano,}
\author[109]{Nathan~Lundblad,}
\author[110]{Cristian~de~J.~López~Monjaraz,}
\author[33,*]{Adam~Lowe,}
\author[88]{Mažena~Mackoit-Sinkevičienė,}
\author[84,104]{Michele~Maggiore,}
\author[111]{Anirban~Majumdar,}
\author[11]{Konstantinos~Makris,}
\author[57]{Azadeh~Maleknejad,}
\author[17]{Anna~L.~Marchant,}
\author[66]{Agnese~Mariotti,}
\author[15]{Christos~Markou,}
\author[28]{Barnaby~Matthews,}
\author[112]{Anupam~Mazumdar,}
\author[57,*]{Christopher~McCabe,}
\author[10]{Matthias~Meister,}
\author[21]{Giorgio~Mentasti,}
\author[113]{Jonathan~Menu,}
\author[114]{Giuseppe~Messineo,}
\author[92,*]{Bernd~Meyer-Hoppe,}
\author[115]{Salvatore~Micalizio,}
\author[116]{Federica~Migliaccio,}
\author[117]{Peter~Millington,}
\author[50,51]{Milan~Milosevic,}
\author[1]{Abhay~Mishra,}
\author[44,*]{Jeremiah~Mitchell,}
\author[118]{Gavin~W.~Morley,}
\author[44]{Noam~Mouelle,}
\author[119]{J\"urgen~M\"uller,}
\author[28,*]{David~Newbold,}
\author[68]{Wei-Tou~Ni,}
\author[1]{Christian~Niehof,}
\author[64]{Johannes~Noller,}
\author[120]{Senad~Od\v{z}ak,}
\author[72]{Daniel~K.~L.~Oi,}
\author[11]{Andreas~Oikonomou,}
\author[121,122,123]{Yasser~Omar,}
\author[124,*]{Chris~Overstreet,}
\author[11]{Vishnupriya~Puthiya~Veettil,}
\author[94]{Julia~Pahl,}
\author[125,*]{Sean~Paling,}
\author[126,*]{Zhongyin~Pan,}
\author[127]{George~Pappas,}
\author[8]{Vinay~Pareek,}
\author[21,*]{Elizabeth~Pasatembou,}
\author[128,129]{Mauro~Paternostro,}
\author[11]{Vishal~K.~Pathak,}
\author[130]{Emanuele~Pelucchi,}
\author[22]{Franck~Pereira~dos~Santos,}
\author[94]{Achim~Peters,}
\author[3]{Annie~Pichery,}
\author[131,132]{Igor~Pikovski,}
\author[117]{Apostolos~Pilaftsis,}
\author[36,85]{Florentina-Crenguta~Pislan,}
\author[133,*]{Robert~Plunkett,}
\author[45]{Rosa~Poggiani,}
\author[134]{Marco~Prevedelli,}
\author[135]{Johann~Rafelski,}
\author[81]{Juhan~Raidal,}
\author[81]{Martti~Raidal,}
\author[3,*]{Ernst~Maria~Rasel,}
\author[136]{S{\' e}bastien~Renaux-Petel,}
\author[137]{Andrea~Richaud,}
\author[11]{Pedro~Rivero-Antunez,}
\author[7]{Tangui~Rodzinka,}
\author[10,*]{Albert~Roura,}
\author[2,133]{Jan~Rudolph,}
\author[22]{Dylan~Sabulsky,}
\author[138,*]{Marianna~S.~Safronova,}
\author[57]{Mairi~Sakellariadou,}
\author[139,*]{Leonardo~Salvi,}
\author[9]{Muhammed~Sameed,}
\author[23]{Sumit~Sarkar,}
\author[1]{Patrik~Schach,}
\author[140]{Stefan~Alaric~Sch{\"a}ffer,}
\author[33]{Jesse~Schelfhout,}
\author[92]{Manuel~Schilling,}
\author[94]{Vladimir~Schkolnik,}
\author[32]{Wolfgang~P.~Schleich,}
\author[3,*]{Dennis~Schlippert,}
\author[44,*]{Ulrich~Schneider,}
\author[23,34,*]{Florian~Schreck,}
\author[141]{Ariel~Schwartzman,}
\author[10]{Nico~Schwersenz,}
\author[142,143]{Olga~Sergijenko,}
\author[144]{Haifa~Rejeb~Sfar,}
\author[145]{Lijing~Shao,}
\author[33,*]{Ian~Shipsey,}
\author[145,146,147]{Jing~Shu,}
\author[43]{Yeshpal~Singh,}
\author[148,149]{Carlos~F.~Sopuerta,}
\author[150]{Marianna~Sorba,}
\author[151]{Fiodor~Sorrentino,}
\author[152]{Alessandro~D.A.M~Spallicci,}
\author[36]{Petruta~Stefanescu,}
\author[127]{Nikolaos~Stergioulas,}
\author[32]{Daniel~Stoerk,}
\author[94]{Hrudya~Thaivalappil~Sunilkumar,}
\author[32]{Jannik~Str{\"o}hle,}
\author[28,*]{Zoie~Tam,}
\author[2]{Dhruv~Tandon,}
\author[44]{Yijun~Tang,}
\author[4]{Dorothee~Tell,}
\author[153]{Jacques~Tempere,}
\author[133]{Dylan~J.~Temples,}
\author[8]{Rohit~P~Thampy,}
\author[94]{Ingmari~C.~Tietje,}
\author[139,*]{Guglielmo~M.~Tino,}
\author[38]{Jonathan~N.~Tinsley,}
\author[36]{Ovidiu~Tintareanu~Mircea,}
\author[44]{Kimberly~Tkalčec,}
\author[21]{Andrew~J.~Tolley,}
\author[116]{Vincenza~Tornatore,}
\author[154]{Alejandro~Torres-Orjuela,}
\author[155]{Philipp~Treutlein,}
\author[18]{Andrea~Trombettoni,}
\author[156]{Christian~Ufrecht,}
\author[81,157,*]{Juan~Urrutia,}
\author[17]{Tristan~Valenzuela,}
\author[133,*]{Linda~R.~Valerio,}
\author[28,*]{Maurits~van~der~Grinten,}
\author[81,114,158]{Ville~Vaskonen,}
\author[145]{Ver\'{o}nica~V\'{a}zquez-Aceves,}
\author[81]{Hardi~Veerm\"ae,}
\author[159]{Flavio~Vetrano,}
\author[160]{Nikolay~~V.~Vitanov,}
\author[11,*]{Wolf~von~Klitzing,}
\author[79]{Sebastian~Wald,}
\author[21,*]{Thomas~Walker,}
\author[161]{Reinhold~Walser,}
\author[68]{Jin~Wang,}
\author[162]{Yan~Wang,}
\author[163,*]{C.~A.~Weidner,}
\author[164]{André~Wenzlawski,}
\author[3]{Michael~Werner,}
\author[92]{Lisa~W{\"o}rner,}
\author[165]{Mohamed~E.~Yahia,}
\author[166]{Efe~Yazgan,}
\author[167]{Emmanuel~Zambrini~Cruzeiro,}
\author[168]{M.~Zarei,}
\author[68,*]{Mingsheng~Zhan,}
\author[44]{Shengnan~Zhang,}
\author[68,*]{Lin~Zhou,}
\author[86,169]{Erik~Zupanič}

% Affiliation List
\affiliation[1]{Technische Universit{\"a}t Darmstadt, Fachbereich Physik, Institut f{\"u}r Angewandte Physik, Schlossgartenstrasse 7, 64289 Darmstadt, Germany}
\affiliation[2]{Department of Physics, Stanford University, Stanford, California 94305, USA}
\affiliation[3]{Leibniz Universit\"at Hannover, Institut f\"ur Quantenoptik, Welfengarten 1, 30167 Hannover, Germany}
\affiliation[4]{Max-Planck-Institut f\"ur Quantenoptik, Hans-Kopfermann-Strasse 1, 85748 Garching, Germany}
\affiliation[5]{Fakult\"at f\"ur Physik, Ludwig-Maximilians-Universit\"at, Schellingstrasse 4, 80799 M\"unchen, Germany}
\affiliation[6]{Munich Center for Quantum Science and Technology (MCQST), Schellingstrasse 4, 80799 M\"unchen, Germany}
\affiliation[7]{Laboratoire Collisions Agr\'{e}gats R\'{e}activit\'{e} UMR5589, University of Toulouse III Paul Sabatier CNRS, 118 Route de Narbonne, Toulouse, FR}
\affiliation[8]{Foundation for Research and Technology-Hellas (FORTH), Heraklion, 70013, Greece}
\affiliation[9]{CERN, CH-1211 Geneva 23, Switzerland}
\affiliation[10]{Institute of Quantum Technologies, German Aerospace Center (DLR), Wilhelm-Runge-Stra\ss{e} 10, 89081 Ulm, Germany}
\affiliation[11]{BEC and Matterwave Optics Group, Institute of Electronic Structure and Lasers, Foundation for Research and Technology - Hellas, Nikolaou Plastira 100, Crete, 70013, GR}
\affiliation[12]{Institute of Physics Belgrade, University of Belgrade, Pregrevica 118, 11080 Belgrade, Serbia}
\affiliation[13]{Serbian Academy of Sciences and Arts, Kneza Mihaila 35, 11000 Belgrade, Serbia}
\affiliation[14]{Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Wilberforce Road, Cambridge, CB3 0WA, UK}
\affiliation[15]{Institute of Nuclear and Particle Physics, NCSR Demokritos, Neapoleos 27 \& Patr. Grigoriou Street, Ag. Paraskevi Attikis, Athens, 15341 Greece}
\affiliation[16]{Department of Civil and Industrial Engineering, University of Pisa, Largo Lucio Lazzarino, Pisa, 56122, Italy}
\affiliation[17]{RAL Space, Rutherford Appleton Laboratory, UKRI-STFC, Fermi Avenue, Didcot, OX11 OQX, UK}
\affiliation[18]{Department of Physics, University of Trieste, Strada Costiera 11, 34151 Trieste, Italy}
\affiliation[19]{Istituto Nazionale di Fisica Nucleare, Trieste Section, Via Valerio 2, 34127 Trieste, Italy}
\affiliation[20]{University of Glasgow, Glasgow G12 8QQ, UK}
\affiliation[21]{Physics Department, Imperial College London, Prince Consort Road, London, SW7 2AZ, UK}
\affiliation[22]{LNE-SYRTE, Observatoire de Paris, Universit\'{e} PSL, CNRS, Sorbonne Universit\'{e}, Paris, France}
\affiliation[23]{Van der Waals-Zeeman Institute, Institute of Physics, University of Amsterdam, Science Park 904, 1098XH Amsterdam, The Netherlands}
\affiliation[24]{Institute of Atomic and Molecular Sciences, Academia Sinica, Taipei 10617, Taiwan}
\affiliation[25]{IFIC, Joint Centre CSIC-University of Valencia,  E-46100 Burjassot, Valencia, Spain}
\affiliation[26]{Laboratoire Photonique, Num\'{e}rique et Nanosciences (LP2N), Universit\'{e} de Bordeaux-IOGS-CNRS, F-33400 Talence, France}
\affiliation[27]{Department of Physics and Astronomy and Institute of Optics, University of Rochester, Rochester, New York, 14627, USA}
\affiliation[28]{STFC Rutherford Appleton Laboratory, Harwell Campus, Didcot, Oxfordshire, OX11 0QX, UK}
\affiliation[29]{Institut de F\'isica d’Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona), Spain}
\affiliation[30]{Instituci\'o Catalana de Recerca i Estudis Avan\c cats (ICREA), Passeig Llu\'is Companys 23, 08010 Barcelona, Spain}
\affiliation[31]{Physics Department, Technion -- Israel Institute of Technology, 3200002, Haifa, Israel}
\affiliation[32]{Institut f{\"u}r Quantenphysik and Center for Integrated Quantum Science and Technology (IQST), Universit{\"a}t Ulm, Albert-Einstein-Allee 11, Ulm D-89081, Germany}
\affiliation[33]{Department of Physics, University of Oxford, Parks Road, Oxford OX1 3PU, UK}
\affiliation[34]{QuSoft, Science Park 123, 1098XG Amsterdam, The Netherlands}
\affiliation[35]{Eindhoven University of Technology, P.O. Box 513, 5600MB Eindhoven, The Netherlands}
\affiliation[36]{Institute of Space Science - INFLPR Subsidiary, 409 Atomistilor street, Magurele, Ilfov, 077125, Romania}
\affiliation[37]{Physics Department, King's College London, Strand, London, WC2R 2LS, UK}
\affiliation[38]{Department of Physics, University of Liverpool, Merseyside L69 7ZE, UK}
\affiliation[39]{Basque Center for Applied Mathematics (BCAM), Alameda de Mazarredo 14, 48009 Bilbao, Spain}
\affiliation[40]{EHU Quantum Center, University of the Basque Country UPV/EHU, Bilbao, Spain}
\affiliation[41]{Department of Physics, University of Crete, Heraklion, 71003, Greece}
\affiliation[42]{School of Sciences, European University Cyprus, Diogenes Street, Engomi, 1516 Nicosia, Cyprus}
\affiliation[43]{Cold Atoms Group, School of Physics and Astronomy, University of Birmingham, Edgbaston, Birmingham B15 2TT, UK}
\affiliation[44]{Cavendish Laboratory, University of Cambridge, J. J. Thomson Avenue, Cambridge CB3 0HE, UK}
\affiliation[45]{Department of Physics ``Enrico Fermi'', University of Pisa, Largo Bruno Pontecorvo 3, 56126 Pisa, Italy}
\affiliation[46]{INFN-Pisa, Largo Bruno Pontecorvo 3, 56126 Pisa, Italy}
\affiliation[47]{Laboratoire Kastler Brossel, Sorbonne Universit\'{e}, CNRS, ENS-Universit\'{e} PSL, Coll\`{e}ge de France, 4 place Jussieu, 75005 Paris, France}
\affiliation[48]{Univ. Lille, CNRS, UMR 8523 - PhLAM - Physique des Lasers Atomes et Mol\'{e}cules, F-59000 Lille, France}
\affiliation[49]{Department of Physics, University of Michigan, Ann Arbor, MI, USA, 48109}
\affiliation[50]{Department of Physics, University of Nis, Serbia}
\affiliation[51]{SEENET-MTP Centre, Nis, Serbia}
\affiliation[52]{Max-Planck-Institut f\"{u}r Physik, Boltzmannstrasse 8, 85748 Garching, Germany}
\affiliation[53]{Institute of Electronic Structure and Laser, Foundation for Research and Technology – Hellas, Heraklion, Greece}
\affiliation[54]{Department of Physics and Astronomy, University of Sussex, Brighton, BN1 9QH, UK}
\affiliation[55]{Department of Physics and Joint Quantum Institute, University of Maryland, College Park, MD 20742, USA}
\affiliation[56]{The Oskar Klein Centre, Department of Physics, Stockholm University, 10691 Stockholm, Sweden}
\affiliation[57]{Physics~Department, King's~College~London, Strand, London, WC2R~2LS, UK}
\affiliation[58]{Gravity Exploration Institute, School of Physics and Astronomy, Cardiff University, Cardiff, CF24 3AA, United Kingdom}
\affiliation[59]{School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\affiliation[60]{Faculty of Science, Mohammed V University, Avenue des Nations Unies, Agdal, B.P. 8007 N.U., 10000 Rabat, Morocco}
\affiliation[61]{Laboratoire de physique de l’ENS, Ecole Normale Sup\'erieure-PSL, CNRS, Sorbonne Universit\'e, Universit\'e Paris Cit\'e, 24 rue Lhomond, 75231 Paris Cedex 05, France}
\affiliation[62]{Ecole polytechnique, IPP, Palaiseau, France}
\affiliation[63]{School of Science, Shenzhen Campus of Sun Yat-sen University, Shenzhen 518107, China}
\affiliation[64]{Department of Physics \& Astronomy, University College London , London WC1E 6BT, United Kingdom}
\affiliation[65]{School of Physics and Astronomy, University of Southampton, Highfield, Southampton SO17 1BJ, UK}
\affiliation[66]{Institute of Theoretical Physics, Leibniz University Hannover, Appelstrasse 2, 30167 Hannover, Germany}
\affiliation[67]{Physikalisch-Technische Bundesanstalt (PTB), Bundesallee 100, 38116 Braunschweig, Germany}
\affiliation[68]{State Key Laboratory of Magnetic Resonance and Atomic and Molecular Physics,  Wuhan Institute of Physics and Mathematics, Innovation Academy for Precision Measurement Science and Technology, Chinese Academy of Sciences, Wuhan 430071, China}
\affiliation[69]{Department of Physics and Astronomy, University of Kentucky, Lexington, KY 40506-0055, USA}
\affiliation[70]{National Physical Laboratory, Hampton Road, Teddington, TW11 0LW, UK}
\affiliation[71]{Department of Physics and Astronomy and Center for Fundamental Physics, Northwestern University, Evanston, IL, USA}
\affiliation[72]{SUPA and Department of Physics, University of Strathclyde, Glasgow, G4 0NG, United Kingdom}
\affiliation[73]{National Conservatory of Arts and Crafts, 292 Rue Saint-Martin, 75003 Paris}
\affiliation[74]{Department of Physics, University of Washington, Seattle, Washington 98195, USA}
\affiliation[75]{School of Physics and Astronomy, University of Nottingham, University Park, Nottingham, NG7 2RD, UK}
\affiliation[76]{Kavli Institute for Cosmology and Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge, CB3 0HA, UK}
\affiliation[77]{ZARM Center of Applied Space Technology and Microgravity, Universit{\"a}t Bremen, Bremen, Germany}
\affiliation[78]{Department of Physics and Technology, University of Bergen, Allegaten 55, 5007 Bergen, Norway}
\affiliation[79]{Institute of Science and Technology Austria, Klosterneuburg, Austria}
\affiliation[80]{Department of Physics, National Tsing Hua University, Hsinchu, 30013, Taiwan (R.O.C.)}
\affiliation[81]{Keemilise ja bioloogilise f\"u\"usika instituut, R\"avala pst. 10, 10143 Tallinn, Estonia}
\affiliation[82]{Dipartimento di Fisica, Sapienza Universit\`{a} di Roma, Piazzale Aldo Moro 5, 00185, Roma, Italy}
\affiliation[83]{INFN, Sezione di Roma, Piazzale Aldo Moro 2, 00185, Roma, Italy}
\affiliation[84]{Gravitational Wave Science Center (GWSC), Universit\'e de Gen\`eve, CH-1211 Geneva, Switzerland}
\affiliation[85]{Faculty of Physics, University of Bucharest, 405 Atomistilor Street, Magurele, Ilfov, 077125, Romania}
\affiliation[86]{Jo\v{z}ef Stefan Institute, Jamova 39, SI-1000 Ljubljana, Slovenia}
\affiliation[87]{Department of Physics, University of Zurich, Winterthurerstrasse 190, 8057 Zurich, Switzerland}
\affiliation[88]{Institute of Theoretical Physics and Astronomy, Vilnius University, Saul\.etekio 3, LT-10257, Vilnius, Lithuania}
\affiliation[89]{TOPTICA Photonics AG, Lochhamer Schlag 19 82166 Graefelfing (Munich), Germany}
\affiliation[90]{Helsinki Institute of Physics, University of Helsinki, Helsinki, Finland}
\affiliation[91]{Physics Division, School of Applied Mathematical and Physical Sciences, NTUA, Hroon Polytechniou 9, 15780, Athens Greece}
\affiliation[92]{Deutsches Zentrum f\"ur  Luft- und Raumfahrt e.V. (DLR), Institut f\"ur  Satellitengeod{\"a}sie und Inertialsensorik, Callinstra{\ss}e 30b, 30167 Hannover, Germany}
\affiliation[93]{D\'{e}partement d'astrophysique, g\'{e}ophysique et oc\'{e}anographie (AGO), L'Universit\'{e} de Li\`{e}ge, Li\`{e}ge, Belgium}
\affiliation[94]{Institut f\"{u}r Physik and IRIS, Humboldt-Universit\"{a}t zu Berlin, Newtonstrasse 15, 12489 Berlin, Germany}
\affiliation[95]{Ferdinand-Braun-Institut (FBH), Gustav-Kirchoff-Strasse 4, 12489 Berlin, Germany}
\affiliation[96]{School of Physics and Institute for Collider Particle Physics, University of the Witwatersrand, Johannesburg, Wits 2050, South Africa.}
\affiliation[97]{Experimental Condensed Matter Physics Group, Ultrafast Coherent Spectroscopy Laboratory, Indian Institute of Science Education and Research, Bhopal, 462066, India}
\affiliation[98]{Center for Quantum Science and Engineering, National Taiwan University, Taipei 10617, Taiwan}
\affiliation[99]{Brown University, Dept. of Physics, 182 Hope St., Providence, RI 02912, USA}
\affiliation[100]{Jet Propulsion Laboratory, California Institute of Technology, Pasadena, California 91109, USA}
\affiliation[101]{Centre for Cold Matter, Blackett Laboratory, Imperial College, Prince Consort Road, London, SW7 2AZ, UK}
\affiliation[102]{European Space Agency (ESA), European Centre for Space Applications and Telecommunications (ECSAT), Fermi Avenue, Harwell Campus, Didcot, OX11 0FD, UK}
\affiliation[103]{Faculty of Physics, University of Warsaw, ul. Pasteura 5, 02-093 Warsaw, Poland}
\affiliation[104]{D\'epartement de Physique Th\'eorique, Universit\'e de Gen\`eve, 24 quai Ernest Ansermet, 1211 Gen\`eve 4, Switzerland}
\affiliation[105]{Departamento de F{\' i}sica Te{\' o}rica, Universidad Aut{\' o}noma de Madrid, 28049 Madrid, Spain}
\affiliation[106]{Instituto de Fisica Teorica UAM-CSIC, 28049 Madrid, Spain}
\affiliation[107]{Department of Mathematics and Physics, Autonomous University of Aguascalientes, Av. Universidad 940, Aguascalientes 20100, Mexico}
\affiliation[108]{Department of Chemistry, Physics and Environmental and Soil Sciences, Escola Politecninca Superior, Universidad de Lleida, Av. Jaume II, 69, 25001 Lleida, Spain}
\affiliation[109]{Department of Physics and Astronomy, Bates College, Lewiston, Maine, USA}
\affiliation[110]{Centro de Investigaci\'{o}n y de Estudios Avanzados del I. P. N., Unidad Quer\'{e}taro, Libramiento Norponiente No. 2000, Fracc. Real de Juriquilla, C. P. 76230, Quer\'{e}taro, Qro., Mexico}
\affiliation[111]{Department of Physics, Indian Institute of Science Education and Research - Bhopal, Bhopal Bypass Road, Bhauri, Bhopal 462066, Madhya Pradesh, India}
\affiliation[112]{Van Swinderen Institute, University of Groningen, 9747 AG, Netherlands}
\affiliation[113]{Institute for Theoretical Physics, KU Leuven, Celestijnenlaan 200D, 3001 Leuven, Belgium}
\affiliation[114]{Istituto Nazionale di Fisica Nucleare, Sezione di Padova, Via Marzolo 8, 35131 Padova, Italy}
\affiliation[115]{Quantum Metrology and Nanotechnologies Division, INRIM, Strada delle Cacce 91, 10135 Torino, Italy}
\affiliation[116]{Politecnico di Milano, DICA, Piazza Leonardo da Vinci, 32, Milan, 20133, IT}
\affiliation[117]{Department of Physics and Astronomy, University of Manchester, Manchester M13 9PL, UK}
\affiliation[118]{Department of Physics, University of Warwick, Coventry CV4 7AL, UK}
\affiliation[119]{Leibniz University Hannover, Institute of Geodesy, Schneiderberg 50, 30167 Hannover, Germany}
\affiliation[120]{University of Sarajevo - Faculty of Science, Zmaja od Bosne 33-35, 71000 Sarajevo, Bosnia and Herzegovina}
\affiliation[121]{Instituto Superior Técnico, Universidade de Lisboa, Portugal}
\affiliation[122]{Physics of Information and Quantum Technologies Group, Centro de Física e Engenharia de Materiais Avançados (CeFEMA), Portugal}
\affiliation[123]{PQI -- Portuguese Quantum Institute, Portugal}
\affiliation[124]{Department of Physics and Astronomy, The Johns Hopkins University, Baltimore, MD 21218, USA}
\affiliation[125]{Boulby Underground Laboratory, Boulby Mine, Saltburn-by-the-Sea, TS13 4UZ, UK}
\affiliation[126]{Technology, Science and Technology Facilities Council, Harwell Campus, Didcot, OX11 0QX, UK}
\affiliation[127]{Department of Physics, Aristotle University of Thessaloniki, Thessaloniki 54124, Greece}
\affiliation[128]{Universit{\` a} degli Studi di Palermo, Dipartimento di Fisica e Chimica - Emilio Segr{\` e}, via Archirafi 36, I-90123 Palermo, Italy}
\affiliation[129]{Centre for Quantum Materials and Technologies, School of Mathematics and Physics, Queen’s University Belfast, BT7 1NN, United Kingdom}
\affiliation[130]{Epitaxy and Physics of Nanostructures, Tyndall National Institute, University College Cork, Lee Maltings, Dyke Parade, Cork, T12R5CP, Ireland}
\affiliation[131]{Department of Physics, Stevens Institute of Technology, One Castle Point Terrace, Hoboken, NJ 07030, USA}
\affiliation[132]{Fysikum, Stockholm University, AlbaNova University Center, 106 91 Stockholm, Sweden}
\affiliation[133]{Fermi National Accelerator Laboratory, POB 500, Batavia, IL 60510, USA}
\affiliation[134]{Department of Physics and Astronomy, University of Bologna, Viale Berti-Pichat 6/2, Bologna, 40126, Italy}
\affiliation[135]{Department of Physics, The University of Arizona, Tucson, AZ 85721-0081, USA}
\affiliation[136]{Institut d’Astrophysique de Paris, CNRS and Sorbonne Universit\'{e}, 98 bis bd Arago, 75014 Paris, France}
\affiliation[137]{Departament de F\'isica, Universitat Polit\`ecnica de Catalunya, Campus Nord B4-B5, E-08034 Barcelona, Spain}
\affiliation[138]{Department of Physics and Astronomy, University of Delaware, Delaware 19716, USA}
\affiliation[139]{Dipartimento di Fisica e Astronomia and LENS, Universit\`{a} di Firenze, INFN Sezione di Firenze, via Sansone 1, I-50019 Sesto Fiorentino (FI), Italy}
\affiliation[140]{Niels Bohr Institute, University of Copenhagen, Blegdamsvej 17, Copenhagen, 2100, DK}
\affiliation[141]{SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, California 94025, USA}
\affiliation[142]{Main Astronomical Observatory of the National Academy of Sciences of Ukraine, Zabolotnoho str., 27, 03143, Kyiv, Ukraine}
\affiliation[143]{AGH University of Krakow, Aleja Mickiewicza, 30, 30-059, Krakow, Poland}
\affiliation[144]{Department of Physics, University at Buffalo, State University of New York, Fronczak Hall, 239, Buffalo, NY 14260, USA}
\affiliation[145]{Kavli Institute for Astronomy and Astrophysics, Peking University, Beijing 100871, China}
\affiliation[146]{School of Physics and State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, China}
\affiliation[147]{Beijing Laser Acceleration Innovation Center, Huairou, Beijing, 101400, China}
\affiliation[148]{Institut de Ci\`encies de l'Espai (ICE-CSIC), Campus UAB, Carrer de Can Magrans~s/n, Cerdanyola del Vall\`es~08193, Spain}
\affiliation[149]{Institut d'Estudis Espacials de Catalunya (IEEC), Edifici RDIT, C/ Esteve~Terradas, 1, desp.~212, Castelldefels~08860, Spain}
\affiliation[150]{SISSA, Via Bonomea 265, 34136 Trieste, Italy}
\affiliation[151]{Sezione di Genova, Istituto Nazionale di Fisica Nucleare, Genova, Italy}
\affiliation[152]{Universit\'e d’Orl\'eans, Laboratoire de Physique et Chimie de l’Environnement et de l’Espace, 3A Avenue de la Recherche Scientifique, 45071 Orl\'eans, France}
\affiliation[153]{TQC, Physics Department, Universiteit Antwerpen, Universiteitsplein 1, Antwerpen, B-2610, Belgium}
\affiliation[154]{Beijing Institute of Mathematical Sciences and Applications, Beijing 101408, China}
\affiliation[155]{Department of Physics, University of Basel, Klingelbergstrasse 82, 4056 Basel, Switzerland}
\affiliation[156]{Self-Learning Systems Group, Fraunhofer IIS, Nuremberg, Bavaria, Germany}
\affiliation[157]{Departament of Cybernetics, Tallinn University of Technology, Akadeemia tee 21, 12618 Tallinn, Estonia}
\affiliation[158]{Dipartimento di Fisica e Astronomia, Universit\`a degli Studi di Padova, Via Marzolo 8, 35131 Padova, Italy}
\affiliation[159]{Virgo Group, DiSPeA, Carlo Bo University, Via S.Chiara 27, Urbino, PU 61029, Italy}
\affiliation[160]{Center for Quantum Technologies, Faculty of Physics, Sofia University, 5 James Bourchier blvd., 1164 Sofia, Bulgaria}
\affiliation[161]{Institute for Applied Physics, Technical University of Darmstadt, Darmstadt, Hassia, Germany}
\affiliation[162]{School of Civil, Aerospace and Design Engineering, University of Bristol, Bristol, BS81TR, UK}
\affiliation[163]{Quantum Engineering Technology Laboratories, H. H. Wills Physics Laboratory and Department of Electrical and Electronic Engineering, University of Bristol, Bristol BS8 1FD, UK}
\affiliation[164]{Johannes Gutenberg University, Staudingerweg 7, 55128 Mainz, Germany}
\affiliation[165]{Abu Dhabi Polytechnic, Institute of Applied Technology, Abu Dhabi 111499, UAE}
\affiliation[166]{Department of Physics, National Taiwan University, No.1 Sec.4 Roosevelt Road Taipei 10617,Taiwan}
\affiliation[167]{Instituto de Telecomunica\c{c}ões, Av. Rovisco Pais 1, 1049-001, Lisboa, Portugal}
\affiliation[168]{Department of Physics, Isfahan University of Technology, 84156-83111 Isfahan, Iran}
\affiliation[169]{AtomQL, Ajdovscina 1, SI-1000 Ljubljana, Slovenia}

